Explainable Planning for Hybrid Systems

The recent advancement in artificial intelligence (AI) technologies facilitates a paradigm shift toward automation. Autonomous systems are fully or partially replacing manually crafted ones. At the core of these systems is automated planning. With the advent of powerful planners, automated planning is now applied to many complex and safety-critical domains, including smart energy grids, self-driving cars, warehouse automation, urban and air traffic control, search and rescue operations, surveillance, robotics, and healthcare. There is a growing need to generate explanations of AI-based systems, which is one of the major challenges the planning community faces today. The thesis presents a comprehensive study on explainable artificial intelligence planning (XAIP) for hybrid systems that capture a representation of real-world problems closely.

==> Chapters/Chapter2/abstract.tex <==
\begin{abstract}
\noindent
In artificial intelligence planning, having an explanation of a plan given by a planner is often desirable. The ability to explain various aspects of a synthesized plan to an end-user not only brings in trust on the planner but also reveals insights of the planning domain and the planning process. Contrastive questions such as “Why action A instead of action B?” can be answered with a contrastive explanation that compares properties of the original plan containing A against the contrastive plan containing B. In this paper, we explore a set of contrastive questions that a user of a planning tool may raise and we propose a \emph{re-model and re-plan} framework to provide explanations to such questions. Earlier work has reported this framework on planning instances for discrete problem domains described in the Planning Domain Definition Language (PDDL) and its variants. In this paper, we propose an extension for planning instances described by PDDL+ for hybrid systems which portray a mix of discrete-continuous dynamics. Specifically, given a mixed discrete continuous system model in PDDL+ and a plan describing the set of desirable actions on the same to achieve a destined goal, we present a framework that can integrate contrastive questions in PDDL+ and synthesize alternate plans. We present a detailed case study on our approach and propose a comparison metric to compare the original plan with the alternate ones. 
\end{abstract}

==> Chapters/Chapter2/acknowledgement.tex <==
\subsection{Acknowledgements}
\noindent The authors would like to acknowledge Swarup Mohalik and Ramamurthy Badrinath, Ericsson Research Bangalore, for initial discussions that led to this problem description. Mir Md Sajid Sarwar and Rajarshi Ray are supported by the Science and Engineering Research Board (SERB) project with File No. IMP/2018/000523.

==> Chapters/Chapter4/abstract.tex <==
\begin{abstract}
    A recent problem of interest in Explainable AI Planning is that of explaining the unsolvability of planning problems. Though there has been a lot of research on generating explanations of solutions to planning problems, explaining the absence of solutions remains a largely open and understudied problem. %, even though such situations can be the hardest to understand or debug.
    Model reconciliation has been a popular approach for generating explanations for such problems in recent literature, which 
    involves an AI agent and a human planner, who have different models of the planning domain and each explains to the other the 
    differences they have in their domain representations and attempt to arrive at a consensus. More often than not, it is assumed 
    that the AI agent has a correct and complete view of the domain, of which the human only has a partial view. Through 
    reconciliation, the human domain is updated to be consistent with what the AI agent has. Most of the works in this direction are targeted toward classical planning problems on domains represented typically as discrete state transition systems or variants.
    In this work, we provide an approach towards  model reconciliation for planning problems in hybrid systems represented as a 
    mix of discrete and continuous domains. %through \emph{continuous model reconciliation}. 
    %We assume the AI agent and human have domain and task models of the planning problem of a hybrid system that significantly defer from each other. 
    We assume that the agent has a complete model of the environment, while the human has a partial or erroneous model and expects a plan for the planning problem when there is none. The explanation problem is presented as a process of continuous reconciliation between these two entities (agent and human) to make the human domain consistent with that of the agent. 
    %A plan is mapped to a path of a hybrid system which is encoded as a set of linear constraints using linear programming (LP).
    To this effect, we use a mix of graph traversal and path analysis, along with Linear programming to carry out the 
    reconciliation process. In particular, we use the concept of Irreducible Infeasible Sets (IIS) to generate 
    explanations. Experimental results on 2 representative hybrid domains show the efficacy of our approach. 
    %As the irreducible infeasible set (IIS) technique can be deployed on a set of unsatisfiable constraints of an LP to find a minimal set of inconsistent constraints, in this work we provide a method consisting of a discrete path analysis and a path-oriented reachability analysis leveraged with IIS technique to find the invalid transitions and IIS path-segments of the hybrid system as reasons of unsolvability of the planning problem.
    %\textcolor{teal}{These invalid transitions and IIS path-segments can be used to form explanation types such as MPE, PPE, and MCE to reconcile the human model with the agent model for the unsolvability of the planning problem.}
    %These invalid transitions and IIS path-segments can be used to reconcile the human model with the agent model to serve as explanation for the unsolvability of the planning problem.
    %As the irreducible infeasible subset (IIS) technique can be deployed on the unsatisfiable constraint set of the planning problem to give a quick analysis, we show that finding the minimal reconciliation set (MRS) by hitting set construction among the IISs presents a way to reconcile the human model with the agent model to serve as explanation for the unsolvability of the problem.
    
\end{abstract}

==> Chapters/Chapter5/abstract.tex <==
\begin{abstract}
Explaining unsolvability of planning problems is of significant research interest in Explainable AI Planning. A number of research efforts on generating explanations of solutions to planning problems have been reported in AI planning literature. However, explaining the unsolvability of planning problems remains a largely open and understudied problem.
A widely practiced approach to plan generation in the planning community is to decompose planning tasks into sub-problems that help progressively converge towards the ultimate goal. In this work, we propose to adopt the same philosophy of sub-problem identification as an efficient mechanism for analyzing and explaining unsolvability of planning problems in hybrid systems. In particular, for a given unsolvable planning problem, we propose to identify common waypoints, which are universal obstacles to plan existence, in other words, they appear on every path on every plan from the source to the planning goal. This work envisions such waypoints as sub-problems of the planning problem and the unreachability of any of these waypoints as an explanation for the unsolvability of the original planning problem. We propose a novel method of waypoint identification by casting the problem as an instance of the longest common subsequence problem, a widely popular problem in computer science, typically considered as an illustrative example for the dynamic programming paradigm. 
Once the waypoints are identified, we perform symbolic reachability analysis on them to identify the earliest unreachable waypoint and report it as the explanation of unsolvability. We present experimental results on some unsolvable planning problems in hybrid domains. 
\end{abstract}

%In this work, we provide a framework for constructing sub-goals for an unsolvable planning problem through a classical computer science approach of finding the longest common subsequence (lcs) of $n$ strings. 
%We represent the planning domain as a graph structure where we enumerate all source-to-goal paths. We consider these paths as strings and find all the common waypoints that appear in every path by computing the lcs of these path-strings.

==> Chapters/Chapter5/acknowledgement.tex <==
\section{Acknowledgements}
\noindent We would like to acknowledge Sk Asif Iqbal, MS student, Indian Association for the Cultivation of Science, Kolkata, for helping us create problem instances of \emph{Warehouse automation} through an automatic model generation tool. %Mir Md Sajid Sarwar and Rajarshi Ray are supported by the Science and Engineering Research Board (SERB) project with File No. IMP/2018/000523.

==> Chapters/Chapter5/prelims.tex <==
\section{Preliminaries} \label{ch5prelims}

We begin with a formal definition of hybrid automation \cite{ALUR19953,10.1007/3-540-57318-6_30}:

\begin{definition} \label{def:HA}
A hybrid automaton (HA) is a seven tuple HA=\big(\emph{Loc}, \emph{Var}, \emph{Flow}, \emph{Init}, \emph{Lab}, \emph{Edge}, \emph{Inv}\big) where:
\begin{itemize}
    \item \emph{Loc} is a finite set of vertices called locations.
    \item \emph{Var} is a finite set of real-valued variables. A valuation $v$ is an assignment of a real-value to each variable $x \in$ \emph{Var}. We write $V$ for the set of all valuations.
    \item \emph{Flow} is a mapping from each location $l \in \emph{Loc}$ to a set of differential equations $\{\dot{x} = f(x_1,\ldots,x_{|Var|}) \mid x \in \emph{Var}\}$, where $\dot{x}$ denotes the rate of change of variable $x$.
    \item \emph{Init} is a tuple $\langle l_{0}, S \rangle$ such that $l_{0} \in \emph{Loc}$ and $S \subseteq V$.
    \item \emph{Lab} is a finite set of labels.
    \item \emph{Edge} is a finite set of transitions $e = (l, a, g, r, l’)$, each consisting of a source location $l \in \emph{Loc}$, a target location $l'\in \emph{Loc}$, a label $a\in \emph{Lab}$, a guard $g \subseteq V$ and a reset map $r: \mathbb{R}^{|Var|} \to \mathbb{R}^{|Var|}$.
    \item \emph{Inv} is a mapping from each location $l\in \emph{Loc}$ to a subset of valuations $V$. $\Box$
\end{itemize}
\end{definition}

\noindent In the planning context, a transition $e \in \emph{Edge}$ depicts an action $act$ of the domain. The name of the action is the transition's label $e.a$, the pre-condition is the transition's guard $e.g$, and the post-condition is the transition's reset $e.r$. 
%The \emph{Init} of the automaton models the region from which an initial state $I$ of the $Prob$ can be chosen. 
The \emph{Init} of the automaton defines the initial condition of the planning problem. 
The change in the discrete state of the domain due to the action is captured through the transition's source and target location $e.l$ and $e.l’$ respectively. A state of a \emph{HA} is a pair $(l,v)$ consisting of a location $l \in$ Loc and a valuation $v\in V$. $l$ denotes the discrete state whereas $v$ denotes the continuous state of the system. A state can change either due to an application of an action or due to the passage of time following the continuous flow dynamics. The continuous state change is given by $flow_{l}(v, t)$ which is the solution of the differential equation Flow($l$). We refer the former as \emph{action-transition} and the later as \emph{timed-transition}.

A planning problem for a hybrid system consists of a hybrid automaton representation of the planning domain and a problem description which is defined as:
\begin{definition} \label{ch5def:planning_problem}
A \emph{planning problem} $\Pi$ for a hybrid system HA is a pair $(Dom, Prob, Depth)$, where
\begin{itemize}
  \item $Dom$ is represented as a hybrid automation HA defining the planning domain \cite{DBLP:journals/tecs/SarwarRB23}.
  \item $Prob$ is a tuple $\langle Init, Goal\rangle$ representing a problem description, where $Init$ and $Goal$ define the initial and the goal states. $Init$ is a tuple $\langle l_{init}, S_{init} \rangle$ such that $l_{init} \in Loc$ and $S_{init} \subseteq V$ and $Goal$ is a tuple $\langle l_{goal}, S_{goal} \rangle$ such that $l_{goal} \in Loc$ and $S_{goal} \subseteq V$. 
  \item \emph{Depth} $D$ defines the bound on the length of a plan.
  $\Box$
\end{itemize}
\end{definition}


\begin{definition}\label{ch5def:plan}
A plan $\phi$ is a tuple $\langle \lambda, makespan \rangle$. For a planning problem with a set of actions $A$, $\lambda$ is a finite set of pairs $\langle t, act \rangle$ {together with the plan \emph{makespan} $\in \mathbb{R}$}. In the pair, $t \in \mathbb{R}^+$ is the time instance of executing the action $act \in A$. The $makespan$ is the overall duration of the plan. $\Box$
\end{definition}

\noindent We define the concept of an abstract graph corresponding to a hybrid automaton obtained by abstracting out the continuous dynamics and considering only the location-location edge relationship. %from which we extract an initial-goal path.
\begin{definition}
For a hybrid automaton HA = \big(\emph{Loc}, \emph{Var}, \emph{Flow}, \emph{Init}, \emph{Lab}, \emph{Edge}, \emph{Inv}\big), the graph of the automaton is defined as $G_{HA}$ = (Loc, $E$) where $E \subseteq \emph{Loc} \times \emph{Loc}$ such that for every ($l$, $a$, $g$, $r$, $l'$) $\in \emph{Edge}$, there is an edge ($l$, $l'$) $\in E$. $\Box$
\end{definition}

\noindent For an abstract graph $\mathcal{G_{HA}}$ corresponding to a hybrid automaton $\mathcal{HA}$, we extract a path $p$ from $\mathcal{G_{HA}}$. In this graph, a path is a plan from the initial location to the goal location in the domain $Dom$ specified in the planning problem $\Pi$. We now define the structure of a path.
\begin{definition}
    A path $p$ in $\mathcal{G_{HA}}$ is a sequence of $vertices$ and $edges$ 
    \begin{align*}
    l_0 \xrightarrow{e_0} l_1 \xrightarrow{e_1} l_2 \xrightarrow{e_2} \ldots \xrightarrow{e_{n-1}} l_N
    \end{align*}
    where $l_i$ $\in$ $Loc$, $e_i$ $\in$ $Edge$, $l_{i} = e_i.l$, $l_{i+1} = e_i.l’$. %and $\sum_{i=0}^{n-1}\tau_{i}$ = \emph{makespan.} 
    $\Box$
\end{definition}

\noindent Corresponding to a path $p$ in $\mathcal{G_{HA}}$, we define the notion of a corresponding {\em run} in $\mathcal{HA}$.
\begin{definition}\label{ch5def:run}
A run corresponding to a path $l_0 \xrightarrow{e_0} l_1 \xrightarrow{e_1} l_2 \xrightarrow{e_2} \ldots \xrightarrow{e_{n-1}} l_N$ 
is an alternating sequence of timed and action transitions of the hybrid automaton depicted as:
\begin{align*}
(l_{0},v_{0}) & \xrightarrow{\tau_0}(l_{0},v'_0) \xrightarrow{e_0} (l_1,v_{1}) \xrightarrow{\tau_1} (l_1,v'_{1})\xrightarrow{e_1} \\
& \ldots, \xrightarrow{e_{n-1}}(l_{n},v_n)\xrightarrow{\tau_{n}} (l_{n},v'_{n})
\end{align*}
where (i) $v_0 \in S$, (ii) $e_i \in Edge$ such that $l_{i} = e_i.l$, $l_{i+1} = e_i.l’$, $v'_{i} \in e_i.g$, $v_{i+1} = e_i.r(v_{i})$, $\forall i \in \{0,\ldots,n-1\}$.
%for all $i=0,\ldots,N-1$ 
%(ii) $e_i(l) = \ell_{i}$ and $e_i(l') = \ell_{i+1}$;
%(i) in each step $i$, $e_i(\ell)$ and $e_i(\ell')$, where $\ell_{i},\ell_{i+1} \in Loc$.
(ii) $\forall t\in [0, \tau_i]$, $flow_{l_i}(v_i, t) \in \emph{Inv}(l_i)$, $\forall i \in \{0,\ldots,n\}$.
(iii) $flow_{l_i}(v_i,\tau_i) = v'_i$;
%(v) $Z_i \in e_i(g)$;
(iv) $v_{i+1} = e_i.r(v_i)$.
%(v) $\sum_{i=0}^{n}{\tau_i}$ = \emph{makespan}.
(vi) $(l_n,v'_n)$ satisfies the goal condition $G$.
$\Box$
\end{definition}

